Interplay of plasmonics and strain for Hexagonal Boron Nitride emission engineering

In the realm of quantum information and sensing, there has been substantial interest in the single-photon emission associated with defects in hexagonal boron nitride (hBN). With the goal of producing deterministic emission centers, in this work, we present a platform for engineering emission in hBN integrated with gold truncated nanocone structures. Our findings highlights that, the activation of emission is due to the truncated gold nanocones. Furthermore, we measure the quantum characteristics of this emission and find that while our system demonstrates support for single-photon emission, the origin of this emission remains ambiguous. Specifically, it is unclear whether the emission arises from defects generated by the induced strain or from alternative defect mechanisms. This uncertainty stems from the fluorescence properties inherent to gold, complicating our definitive attribution of the quantum emission source. To provide a rigorous theoretical foundation, we elucidate the effects of strain via the Kirchhoff-Love theory. Additionally, the enhancements observed due to plasmonic effects are comprehensively explained through the resolution of Maxwell's equations. This study will be useful for the development of deterministic and tunable single photonic sources in two dimensional materials and their integration with plasmonic platforms.

==> biblio.tex <==
\addcontentsline{toc}{section}{Bibliography}
\bibliographystyle{unsrt}
\bibliography{ref.bib}
